AfriSenti: A Twitter Sentiment Analysis Benchmark for African Languages

Africa is home to over 2,000 languages from more than six language families and has the highest linguistic diversity among all continents. These include 75 languages with at least one million speakers each. Yet, there is little NLP research conducted on African languages. Crucial to enabling such research is the availability of high-quality annotated datasets. In this paper, we introduce AfriSenti, a sentiment analysis benchmark that contains a total of >110,000 tweets in 14 African languages (Amharic, Algerian Arabic, Hausa, Igbo, Kinyarwanda, Moroccan Arabic, Mozambican Portuguese, Nigerian Pidgin, Oromo, Swahili, Tigrinya, Twi, Xitsonga, and Yor\`ub\'a) from four language families. The tweets were annotated by native speakers and used in the AfriSenti-SemEval shared task (The AfriSenti Shared Task had over 200 participants. See website at https://afrisenti-semeval.github.io). We describe the data collection methodology, annotation process, and the challenges we dealt with when curating each dataset. We further report baseline experiments conducted on the different datasets and discuss their usefulness.

==> sentiment-class-dist.tex <==
\pgfplotstableread[row sep=\\,col sep=&]{
    language & dpositive & dnegative & dneutral & trpositive & trnegative & trneutral & tepositive & tenegative & teneutral\\
    ma & 385 & 360 & 470 & 1758 & 1664 & 2161 & 1144 & 850 & 967\\
    yo & 884 & 443 & 763 & 3542 & 1872 & 3108 & 1918 & 981 & 1617\\
    ts & 96 & 72 & 35 & 384 & 284 & 136 & 121 & 90 & 43\\
    tg & 61 & 215 & 122 & 0 & 0 & 0 & 643 & 970 & 387\\
    ha & 887 & 894 & 896 & 4687 & 4573 & 4912 & 1755 & 1759 & 1789\\
    twi & 183 & 147 & 58 & 1644 & 1315 & 522 & 450 & 353 & 146\\
    ig & 560 & 470 & 811 & 3084 & 2600 & 4508 & 1118 & 943 & 1621\\
    sw & 137 & 48 & 268 & 547 & 191 & 1072 & 224 & 80 & 444\\
    kr & 225 & 287 & 315 & 899 & 1146 & 1257 & 278 & 355 & 393\\
    pcm & 447 & 813 & 21 & 1808 & 3421 & 72 & 1397 & 2326 & 431\\
    am & 333 & 388 & 776 & 1332 & 1548 & 3104 & 438 & 1337 & 224\\
    pt & 171 & 196 & 400 & 681 & 782 & 1600 & 628 & 655 & 2379\\
    or & 154 & 117 & 125 & 0 & 0 & 0 & 462 & 733 & 896\\
    dz & 105 & 223 & 86 & 417 & 892 & 342 & 326 & 474 & 154\\
}\devClassDist


\begin{figure*}
    \centering
    \resizebox{\textwidth}{!}{%
        \begin{tikzpicture}
        \begin{axis}[ybar,
                width=25cm,
                height=15cm,
                ymin=0,
                ymax=5000,        
                ylabel={Number of tweets},
                xlabel={Languages},
                xtick=data,
                symbolic x coords={am, dz, ha, ig, kr, ma, or, pcm, pt, sw, tg, ts, twi, yo},
                major x tick style = {opacity=0},
                minor x tick num = 1,
                minor tick length=2ex,
                legend entries={positive, negative, neutral},
                legend columns=3,
                legend style={draw=none,nodes={inner sep=3pt}},
            ]
        \addplot[draw=black,fill=bblue] table[x index=0,y index=4] \devClassDist;
        \addplot[draw=black,fill=rred] table[x index=0,y index=5] \devClassDist;
        \addplot[draw=black,fill=ggreen] table[x index=0,y index=6] \devClassDist;
        \end{axis}
        \end{tikzpicture}
    }
    \caption{Training Datasets Sentiment Class Distribution}
    \label{fig:train_class_dist}
\end{figure*}

\begin{figure*}
    \centering
    \resizebox{\textwidth}{!}{%
        \begin{tikzpicture}
        \begin{axis}[ybar,
                width=25cm,
                height=15cm,
                ymin=0,
                ymax=1000,        
                ylabel={Number of tweets},
                xlabel={Languages},
                xtick=data,
                symbolic x coords={am, dz, ha, ig, kr, ma, or, pcm, pt, sw, tg, ts, twi, yo},
                major x tick style = {opacity=0},
                minor x tick num = 1,
                minor tick length=2ex,
                legend entries={positive, negative, neutral},
                legend columns=3,
                legend style={draw=none,nodes={inner sep=3pt}},
            ]
        \addplot[draw=black,fill=bblue] table[x index=0,y index=1] \devClassDist;
        \addplot[draw=black,fill=rred] table[x index=0,y index=2] \devClassDist;
        \addplot[draw=black,fill=ggreen] table[x index=0,y index=3] \devClassDist;
        \end{axis}
        \end{tikzpicture}
    }
    \caption{Development Datasets Sentiment Class Distribution}
    \label{fig:dev_class_dist}
\end{figure*}

\begin{figure*}
    \centering
    \resizebox{\textwidth}{!}{%
        \begin{tikzpicture}
        \begin{axis}[ybar,
                width=25cm,
                height=15cm,
                ymin=0,
                ymax=2500,        
                ylabel={Number of tweets},
                xlabel={Languages},
                xtick=data,
                symbolic x coords={am, dz, ha, ig, kr, ma, or, pcm, pt, sw, tg, ts, twi, yo},
                major x tick style = {opacity=0},
                minor x tick num = 1,
                minor tick length=2ex,
                legend entries={positive, negative, neutral},
                legend columns=3,
                legend style={draw=none,nodes={inner sep=3pt}},
            ]
        \addplot[draw=black,fill=bblue] table[x index=0,y index=7] \devClassDist;
        \addplot[draw=black,fill=rred] table[x index=0,y index=8] \devClassDist;
        \addplot[draw=black,fill=ggreen] table[x index=0,y index=9] \devClassDist;
        \end{axis}
        \end{tikzpicture}
    }
    \caption{Test Datasets Sentiment Class Distribution}
    \label{fig:test_class_dist}
\end{figure*}
